A BV-Category of Spacetime Interventions

We use the Chu construction to functorially build BV-categories from duoidal categories, demonstrating that candidate models of BV-logic can be cofreely constructed from a fragment of a model of Retor\'e's sequencing operator. By using this construction to show that the strong Hyland envelope is a BV-category, we find a way to build a canonical model of spatio-temporal relationships between agents in spacetime from any symmetric monoidal category. The concrete physical interpretation of spacetime events in this model as intervention-context pairs resolves deficiencies in previous attempts to give a general categorical semantics to quantum supermaps.

==> figs/giant.tex <==
\begin{tikzcd}[ampersand replacement=\&]
  \& F(a\otimes b)^* \otimes Fa \otimes Fb \ar[d,"\cong"] \ar[dl,"\cong"'] \ar[r,"1\otimes l"] \& F(a\otimes b)^* \otimes F(a\otimes b) \ar[d,"\cong"] \ar[dr,"l"] \ar[rr,"s^{-1}\otimes 1"] \& \& (F(a\otimes b))^* \otimes F(a\otimes b) \ar[dddddd,"\varepsilon"] \\
  F(a\otimes b)^* \otimes Fa \otimes (Fb^*)^* \ar[d,"\cong"'] \ar[r,"1\otimes 1\otimes s"] \& F(a\otimes b)^* \otimes Fa \otimes Fb^{**} \ar[d,"\cong"] \ar[r,"1\otimes l"] \& F(a\otimes b)^* \otimes F(a\otimes b^{**}) \ar[d,"\cong"] \& |[yshift=-1.8em,overlay]| F((a\otimes b)^*\otimes (a\otimes b)) \ar[ddl,"\cong"] \ar[dddd,"F\epsilon"] \& \\
  F(a^*\parr b^*) \otimes Fa \otimes (Fb^*)^* \ar[d,"l\otimes 1"'] \ar[r,"1\otimes 1\otimes s"] \& F(a^*\parr b^*) \otimes Fa \otimes Fb^{**} \ar[d,"l\otimes 1"] \ar[r,"1\otimes l"] \& F(a^*\parr b^*) \otimes F(a \otimes b^{**}) \ar[d,"l"] \& \& \\
  F((a^*\parr b^*)\otimes a) \otimes (Fb^*)^* \ar[d,"F\delta\otimes 1"'] \ar[r,"1\otimes s"] \& F((a^*\parr b^*)\otimes a) \otimes Fb^{**} \ar[d,"F\delta\otimes 1"] \ar[r,"l"] \& F((a^*\parr b^*)\otimes a \otimes b^{**}) \ar[d,"F(\delta\otimes 1)"] \& \& \\
  F((a^*\otimes a)\parr b^*) \otimes (Fb^*)^* \ar[dd,"F(\varepsilon\parr 1)\otimes 1"'] \ar[r,"1\otimes s"] \& F((a^*\otimes a)\parr b^*) \otimes Fb^{**} \ar[d,"F(\varepsilon\parr 1)\otimes 1"] \ar[r,"l"] \& F(((a^*\otimes a)\parr b^*) \otimes b^{**}) \ar[d,"F((\varepsilon\parr 1)\otimes 1)"] \& \& \\
  \& Fb^* \otimes Fb^{**} \ar[r,"l"] \& F(b^*\otimes b^{**}) \ar[r,"F\varepsilon"] \& F(i_\parr) \ar[dr] \& \\
  Fb^* \otimes (Fb^*)^* \ar[rrrr,"\varepsilon"'] \ar[ur,"1\otimes s"] \& \& \& \& i_\parr \\
\end{tikzcd}

==> figs/giant_reverse.tex <==
\begin{tikzcd}
	&&&&& {Fi_{\otimes}^*} \\
	&& {i_{\parr}} && {(Fi_{\otimes})^*} \\
	&& {((Fa)^* \parr Fa)^*} && {F(a^* \parr a)^*} \\
	&&& {(Fa^* \parr Fa)^*} && {F((a^{**} \otimes a^*)^{**})} \\
	& {(Fa)^{**} \otimes (Fa)^*} \\
	&& {(Fa^{*})^{*} \otimes (Fa)^*} & {(Fa^{**} \otimes Fa^*)^{**}} & {F(a^{**} \otimes a^*)^{**}} \\
	{Fa \otimes (Fa)^*} && {Fa^{**} \otimes (Fa)^*} &&& {F(a^{**} \otimes a^*)} \\
	&&& {Fa^{**} \otimes Fa^*} &&& {F(a \otimes a^*)} \\
	&& {Fa \otimes Fa^*}
	\arrow["{l_{o(\parr)}}"', bend right=18, from=1-6, to=2-3]
	\arrow["s"', from=1-6, to=2-5]
	\arrow["{l_{o(\otimes)}^*}"', from=2-5, to=2-3]
	\arrow["{\eta^*}", from=3-3, to=2-3]
	\arrow["{F(\eta)^*}", from=3-5, to=2-5]
	\arrow["{l_{\parr}^*}", from=3-5, to=4-4]
	\arrow["{(s \parr i)^*}"{description}, from=4-4, to=3-3]
	\arrow["{F\eta^*}"', from=4-6, to=1-6]
	\arrow["s", from=4-6, to=3-5]
	\arrow["d"', from=5-2, to=3-3]
	\arrow["{s \otimes i}"', from=5-2, to=6-3]
	\arrow["d"', from=6-3, to=4-4]
	\arrow["{(s \otimes s)^{**}}"', from=6-4, to=4-4]
	\arrow["{l_{\otimes}^{**}}"', from=6-4, to=6-5]
	\arrow["{s^{*}}"', from=6-5, to=3-5]
	\arrow["\epsilon", bend left=24, from=7-1, to=2-3]
	\arrow["{d \otimes i}"', from=7-1, to=5-2]
	\arrow["{Fd \otimes i}", from=7-1, to=7-3]
	\arrow["{i \otimes s}"', from=7-1, to=9-3]
	\arrow["{s \otimes i}"', from=7-3, to=6-3]
	\arrow["Fd"', from=7-6, to=4-6]
	\arrow["d"', from=7-6, to=6-5]
	\arrow["d"', from=8-4, to=6-4]
	\arrow["{i \otimes s}"', from=8-4, to=7-3]
	\arrow["{l_{\otimes}}"', from=8-4, to=7-6]
	\arrow["{F\epsilon}"', bend right=24, from=8-7, to=1-6]
	\arrow["{F(d \otimes i)}"{description}, from=8-7, to=7-6]
	\arrow["{Fd \otimes i}"', from=9-3, to=8-4]
	\arrow["{l_{\otimes}}"', bend right=30, from=9-3, to=8-7]
\end{tikzcd}


